OmniH2O: Universal and Dexterous Human-to-Humanoid Whole-Body Teleoperation and Learning

We present OmniH2O (Omni Human-to-Humanoid), a learning-based system for whole-body humanoid teleoperation and autonomy. Using kinematic pose as a universal control interface, OmniH2O enables various ways for a human to control a full-sized humanoid with dexterous hands, including using real-time teleoperation through VR headset, verbal instruction, and RGB camera. OmniH2O also enables full autonomy by learning from teleoperated demonstrations or integrating with frontier models such as GPT-4. OmniH2O demonstrates versatility and dexterity in various real-world whole-body tasks through teleoperation or autonomy, such as playing multiple sports, moving and manipulating objects, and interacting with humans. We develop an RL-based sim-to-real pipeline, which involves large-scale retargeting and augmentation of human motion datasets, learning a real-world deployable policy with sparse sensor input by imitating a privileged teacher policy, and reward designs to enhance robustness and stability. We release the first humanoid whole-body control dataset, OmniH2O-6, containing six everyday tasks, and demonstrate humanoid whole-body skill learning from teleoperated datasets.

==> setup.tex <==
\section{Real Robot System Setup}
Our entire computation process is conducted onboard, utilizing two Orin NX computers mounted on the back of the H1 robot. The first Orin NX is connected to a ZED camera mounted on the waist of H1, which performs computations to determine H1's own location for positioning. The camera operates at 60 Hz FPS. Additionally, this Orin NX connects via Wi-Fi to our Vision Pro device to continuously receive motion goal information from a human operator. 

The second Orin NX serves as our main control hub. It receives the motion goal information, which it uses as input for our Universal Control Policy. This policy then outputs torque information for each of the robot's motors and sends these commands to the robot. Furthermore, the information for the robot's fingers and wrists does not require inference; it is directly mapped from the Vision Pro data to the corresponding joints on the robot. The policy's computation frequency is set at 50 Hz.

The two Orin NX units are connected via Ethernet, sharing information through a common ROS (Robot Operating System) network. The final commands to H1 are consolidated and dispatched by the second Orin NX. Our entire system has a low latency of only 20 milliseconds.

It's worth noting that we designed the system in this way partly because the ZED camera requires substantial computational resources. By dedicating the first Orin NX to the ZED camera, and the second to policy inference, we ensure that each component operates with optimal performance.
